VIL-100: A New Dataset and A Baseline Model for Video Instance Lane Detection

Lane detection plays a key role in autonomous driving. While car cameras always take streaming videos on the way, current lane detection works mainly focus on individual images (frames) by ignoring dynamics along the video. In this work, we collect a new video instance lane detection (VIL-100) dataset, which contains 100 videos with in total 10,000 frames, acquired from different real traffic scenarios. All the frames in each video are manually annotated to a high-quality instance-level lane annotation, and a set of frame-level and video-level metrics are included for quantitative performance evaluation. Moreover, we propose a new baseline model, named multi-level memory aggregation network (MMA-Net), for video instance lane detection. In our approach, the representation of current frame is enhanced by attentively aggregating both local and global memory features from other frames. Experiments on the new collected dataset show that the proposed MMA-Net outperforms state-of-the-art lane detection methods and video object segmentation methods. We release our dataset and code at https://github.com/yujun0-0/MMA-Net.

==> ToAE.tex <==

We thank all reviewers and ACs for their time and constructive comments.

Both R1 (weak accept) & R2 (strong accept) all agreed our contributions with many positive comments, e.g., "addressing the lane detection using sequences of frames is a good direction for this problem" "annotated dataset is a valuable contribution to the research commnunity", "dataset can be a useful tool for the research community", "diversity of driving conditions: haze, night" "well presented statistics of the dataset" "experiments are pretty comprehensive".

Unfortunately, R3 (weak reject) seems didn't notice that one most important problem in instance-level video lane detection is that lacking sufficient dataset and a network baseline for the development instance-level video lane detection models.  

We sincerely hope AC lets R3 notice that "The addition of a new dataset to support this idea appears sufficiently justified and it can be a useful tool for the
research community." (said by R1), and "An annotated datasets is a valuable contribution to the research community." (said by R2) during the CVPR discussion period.
